Near-optimal Approximate Discrete and Continuous Submodular Function Minimization

In this paper we provide improved running times and oracle complexities for approximately minimizing a submodular function. Our main result is a randomized algorithm, which given any submodular function defined on $n$-elements with range $[-1, 1]$, computes an $\epsilon$-additive approximate minimizer in $\tilde{O}(n/\epsilon^2)$ oracle evaluations with high probability. This improves over the $\tilde{O}(n^{5/3}/\epsilon^2)$ oracle evaluation algorithm of Chakrabarty \etal~(STOC 2017) and the $\tilde{O}(n^{3/2}/\epsilon^2)$ oracle evaluation algorithm of Hamoudi \etal. Further, we leverage a generalization of this result to obtain efficient algorithms for minimizing a broad class of nonconvex functions. For any function $f$ with domain $[0, 1]^n$ that satisfies $\frac{\partial^2f}{\partial x_i \partial x_j} \le 0$ for all $i \neq j$ and is $L$-Lipschitz with respect to the $L^\infty$-norm we give an algorithm that computes an $\epsilon$-additive approximate minimizer with $\tilde{O}(n \cdot \mathrm{poly}(L/\epsilon))$ function evaluation with high probability.

==> lowerbound.tex <==
\section{Lower Bounds}
In this section we show lower bounds against deterministic algorithms for both submodular functions over $[k]^n$ and continuous submodular functions.
It is well-known that even approximately minimizing submodular functions over $\{0,1\}^n$ requires $\Omega(n)$ function calls. Here we show...

In the work of \cite{CLSW17}, they showed that any randomized algorithm for approximate SFM which only has access to gradient calls requires $\Omega(n)$ gradient calls in expectation. We show the same for continuous submodular functions.
